POLITICS: Pretraining with Same-story Article Comparison for Ideology Prediction and Stance Detection

Ideology is at the core of political science research. Yet, there still does not exist general-purpose tools to characterize and predict ideology across different genres of text. To this end, we study Pretrained Language Models using novel ideology-driven pretraining objectives that rely on the comparison of articles on the same story written by media of different ideologies. We further collect a large-scale dataset, consisting of more than 3.6M political news articles, for pretraining. Our model POLITICS outperforms strong baselines and the previous state-of-the-art models on ideology prediction and stance detection tasks. Further analyses show that POLITICS is especially good at understanding long or formally written texts, and is also robust in few-shot learning scenarios.

==> Tables/table_domain_transfor.tex <==
\begin{table}
\centering
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{llrrrrr}
\toprule
\multicolumn{2}{l}{\backslashbox[40mm]{\textbf{Model}}{\textbf{Test Genre}}}    & CongS  & News  & Tweet       & YT & Avg \\
\midrule
\multicolumn{2}{l}{SVM}          & $51.60$       & $51.28$       & $62.17$  & $44.06$   &  $52.28_{\pm0.00}$   \\
\multicolumn{2}{l}{RoBERTa}      & $45.18$ & $57.28$ & $\textbf{65.02}$ & $52.82$ &  $55.08_{\pm1.89}$   \\
\multicolumn{2}{l}{\model + Ideo. Pred.} & $\textbf{63.05}$ & $\textbf{77.89}$ & $62.09$ & $\textbf{61.08}$ & $\textbf{66.03}_{\pm0.94}$ \\
\multicolumn{2}{l}{\model}     & $58.00$ & $67.80$ & $63.35$ & $58.13$ & $61.82_{\pm0.44}$ \\
\bottomrule
\end{tabular}
}
\caption{
Model performance (macro F1 scores, average of three runs) when transferring to unseen text genres. \textbf{Best} results are in bold. \model achieves better performance than SVM and RoBERTa.}
\label{table:genre-transfer}
\end{table}

==> Tables/table_std.tex <==
\begin{table*}
\centering
\resizebox{1.0\linewidth}{!}{%
\begin{tabular}{lcccccccccccccc}
\toprule
\multicolumn{1}{c}{\multirow{3}{*}{\textbf{}}} & \multicolumn{7}{c}{\textbf{Ideology Prediction}} & \multicolumn{5}{c}{\textbf{Stance Detection}} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{\multirow{3}{*}{\pbox{3em}{All \\ std}}} \\
\cmidrule(lr){2-8}
\cmidrule(lr){9-14}

\multicolumn{1}{c}{} & \multicolumn{1}{c}{YT} & \multicolumn{1}{c}{\multirow{2}{*}{CongS}} & \multicolumn{1}{c}{\multirow{2}{*}{HP}} & \multicolumn{1}{c}{\multirow{2}{*}{AllS}} & \multicolumn{1}{c}{YT} & \multicolumn{1}{c}{\multirow{2}{*}{TW}} & \multicolumn{1}{c}{Ideo.}  & \multicolumn{1}{c}{SEval} & \multicolumn{1}{c}{SEval} & \multicolumn{1}{c}{Basil} & \multicolumn{1}{c}{\multirow{2}{*}{VAST}} & \multicolumn{1}{c}{Basil} & \multicolumn{1}{c}{Stan.}  & \multicolumn{1}{c}{} \\
\multicolumn{1}{c}{} & \multicolumn{1}{c}{(cmt.)} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{(user)} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{std} & \multicolumn{1}{c}{(seen)} & \multicolumn{1}{c}{(unseen)} & \multicolumn{1}{c}{(sent.)} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{(art.)} & \multicolumn{1}{c}{std} & \multicolumn{1}{c}{} \\
\midrule
BERT & 1.92 & 1.13 & 1.44 & 0.83 & 1.53 & 2.03 & 0.56 & 1.02 & 1.53 & 3.95 & 0.43 & 3.92 & 1.22 & 0.69 \\
RoBERTa & 0.85 & 0.48 & 3.13 & 1.26 & 4.03 & 1.52 & 0.64 & 0.87 & \textbf{0.77} & 2.55 & \textbf{0.11} & 7.35 & 1.66 & 0.92 \\ 

% \hdashline[5pt/4pt]
\midrule
\multicolumn{15}{l}{\textbf{Our models with triplet loss objective only}} \\

Ideology Obj. & 1.46 & 0.54 & 6.82 & 1.62 & 6.89 & 10.84 & 2.78 & 0.79 & 3.97 & 4.41 & 0.32 & 5.61 & 1.02 & 1.86\\
Story Obj. & 1.05 & 1.21 & 2.64 & 1.68 & 3.18 & 3.29 & 1.31 & 0.38 & 1.19 & 2.51 & 1.29 & 6.76 & 1.67 & 1.01\\
Ideology Obj. + Story Obj. &  0.44 & 0.71 & 3.10 & 2.96 & 2.83 & 1.42 & 0.62 & 0.45 & 1.92 & 1.58 & 1.13 & 7.55 & 1.54 & 0.86\\

\hdashline[5pt/4pt]
\multicolumn{15}{l}{\textbf{Our models with masked language model objective only}} \\
Random &  1.30 & 0.94 & 2.22 & 1.55 & 1.43 & 2.32 & 0.88 & 0.84 & 0.85 & 1.61 & 0.53 & 3.71 & 0.75 & 0.71\\
Upsamp. Ent. &  1.00 & 0.39 & \textbf{0.98} & 1.81 & 2.23 & \textbf{1.07} & \textbf{0.22} & 0.61 & 1.90 & 1.85 & 1.01 & 5.56 & 1.49 & 0.66 \\
Upsamp. Sentiment & 1.12 & 0.96 & 5.68 & 1.09 & 2.70 & 1.30 & 1.12 & 0.51 & 1.22 & 2.31 & 0.62 & 4.91 & 0.71 & 0.78\\
Upsamp. Ent. + Sentiment &  \textbf{0.37} & 0.51 & 3.34 & \textbf{0.61} & 3.56 & 2.07 & 0.74 & 0.71 & 3.93 & 1.08 & 0.73 & 4.95 & 0.69 & 0.66 \\

\hdashline[5pt/4pt]
\model & 0.49 & \textbf{0.31} & 2.10 & 0.83 & \textbf{1.15} & 2.19 & 0.56 & \textbf{0.36} & 1.23 & \textbf{0.97} & 0.60 & \textbf{3.42} & \textbf{0.56} & \textbf{0.19}\\
\bottomrule
\end{tabular}
}
\caption{
\lu{redo}
Standard deviation of neural models on 11 evaluation tasks. 
Tasks are sorted by text length, short to long, within each group. 
``All std'' is the standard deviation of all 11 tasks. 
\textbf{Smallest} standard deviations are in bold. 
\model achieves the smallest std on 5 out of 11 downstream tasks as well as the lowest overall std. 
%
}
\label{table:std}
\end{table*}
